Asset Price Forecasting using Recurrent Neural Networks

This thesis serves three primary purposes, first of which is to forecast two stocks, i.e. Goldman Sachs (GS) and General Electric (GE). In order to forecast stock prices, we used a long short-term memory (LSTM) model in which we inputted the prices of two other stocks that lie in rather close correlation with GS. Other models such as ARIMA were used as benchmark. Empirical results manifest the practical challenges when using LSTM for forecasting stocks. One of the main upheavals was a recurring lag which we called "forecasting lag". The second purpose is to develop a more general and objective perspective on the task of time series forecasting so that it could be applied to assist in an arbitrary that of forecasting by ANNs. Thus, attempts are made for distinguishing previous works by certain criteria (introduced by a review paper written by Ahmed Tealab) so as to summarise those including effective information. The summarised information is then unified and expressed through a common terminology that can be applied to different steps of a time series forecasting task. The last but not least purpose of this thesis is to elaborate on a mathematical framework on which ANNs are based. We are going to use the framework introduced in the book "Neural Networks in Mathematical Framework" by Anthony L. Caterini in which the structure of a generic neural network is introduced and the gradient descent algorithm (which incorporates backpropagation) is introduced in terms of their described framework. In the end, we use this framework for a specific architecture, which is recurrent neural networks on which we concentrated and our implementations are based. The book proves its theorems mostly for classification case. Instead, we proved theorems for regression case, which is the case of our problem.

==> Chapters/Chapter_V.tex <==
\clearpage
\chapter{Conclusion}
\clearpage
Conclusion
In the first chapter, at first we reviewed the works done for the task of stock price prediction and specifically, works that use RNN networks for this task. Then, we pinpointed the research gaps in the papers that use ANNs for the task of time series forecasting. We subsequently distinguished practical articles based on introduced criteria and extracted information form them so as to facilitate future works. The extracted information is pivotal in the steps that should be taken for a time series forecasting task. Hopefully, this will help to achieve a general strategy so that time series forecasting
can be done more objectively instead of a problem-oriented approach which is solely based on the researcher's subjective experience.\\ \\

In chapter 2 we described the general notion of deep learning along with its relation to neural networks. Furthermore, we pinpointed the advantages of deep learning models over traditional machine learning models from different perspectives, one of which was the ideas of representation of data and depth, and another one was reaching the fact that neural networks impose fewer prior beliefs on data in comparison to other models. Afterward, the structure of neural networks was introduced by pinpointing the way they are built upon perceptrons and sigmoid neurons. Then, we elaborated on the structure of RNNs after stressing their significant capability of memorizing earlier input as
well as earlier outputs. We subsequently posed the challenge of long term dependency and proposed approaches to overcome it, such as leaky units and LSTMs. Finally, we described the structure of LSTMs by introducing the concepts of cell-state and gates and then explicate the interaction between the cell-state and the three gates contributing LSTMs (forget, input and output) through a step-by-step walk-through. \\
We realized that before feeding current input and previous state’s output to the current state of the model, an input gate decides which parts of them to be discarded before entering the cell state. Afterward, an input gate looks into the new input and previous output (from which some parts are already discarded) and select the parts of them that are preferred to be stored in the cell state. Before storing new information, a vector of candidate values is created by a tanh layer. Thereafter, the cell state is updated by carrying out the tasks of the forget and output gates. Eventually, before the cell state output its values, an output gate regulates the leakage of information by choosing the parts that are yet to be outputted and serve as a new input for the next state.
This introduction to LSTMs would be insightful for understanding our practical part of this thesis, chapter 3, in which we applied LSTM on stock prices in order to perform one-step ahead forecast, as
well as theoretical part, Chapter 4 in which the mathematical formalization of NNs and especially, RNNs and gated RNNs are explained in section 4.\\ \\

In chapter 3, from reported figures and accuracy as well as the forecasting lag problem, we can conclude that provided that the target feature is price return, the model will be immune to falling into the forecasting lag trap. On the other hand, designating price return as feature is at the expense of the model losing sight of the trends and magnitude of change over time. Consequently, it seems that forecasting stocks’ prices by their historical data as the sole feature by LSTM seems a quite cumbersome and perhaps impossible task due to the mentioned issues. This is in contradiction with the
suggestive theory that LSTM seems like the most suitable model for predicting prices and sequence data in general.\\ \\

In the final chapter, we introduced a mathematical framework on which neural networks can be defined. By dint of this framework, neural networks can be formalized and gradient descent (GD)algorithm (which incorporates backpropagation) is expressed through the framework. At first, the framework was developed for a generic NN and GD was expressed through it. Afterward, we
concentrated on specific structures, from which we chose RNNs. Finally, we narrowed our scope to specific RNN structures, which are Vanilla RNN and LSTM.
